Measuring the Robustness of NLP Models to Domain Shifts

Existing research on Domain Robustness (DR) suffers from disparate setups, limited task variety, and scarce research on recent capabilities such as in-context learning. Furthermore, the common practice of measuring DR might not be fully accurate. Current research focuses on challenge sets and relies solely on the Source Drop (SD): Using the source in-domain performance as a reference point for degradation. However, we argue that the Target Drop (TD), which measures degradation from the target in-domain performance, should be used as a complementary point of view. To address these issues, we first curated a DR benchmark comprised of 7 diverse NLP tasks, which enabled us to measure both the SD and the TD. We then conducted a comprehensive large-scale DR study involving over 14,000 domain shifts across 21 fine-tuned models and few-shot LLMs. We found that both model types suffer from drops upon domain shifts. While fine-tuned models excel in-domain, few-shot LLMs often surpass them cross-domain, showing better robustness. In addition, we found that a large SD can often be explained by shifting to a harder domain rather than by a genuine DR challenge, and this highlights the importance of TD as a complementary metric. We hope our study will shed light on the current DR state of NLP models and promote improved evaluation practices toward more robust models.

==> 6.results_naveh.tex <==
\section{Results}
\label{sec:results}

\input{tables/main_table_ft}
\input{tables/main_table}
\input{figures/scenarios_barplot_tex}
\input{tables/correlations}

In this section, we aim to analyze our extensive experimentation. We start by asking if and under which circumstances the DR exists. We then try to characterize its behavior, and to compare the two points of view presented in \ref{sec:methods}: The source's and the target's. We conclude by comparing the performance and robustness of FT and few-shot models. 

\subsection{Is DR still a challenge?}
\label{sub:dr_challenge}
The vast majority of tasks still exhibit non-negligible drops in performance upon domain transfer of fine-tuned models. An exception to this is the QA and QG tasks, which share the same partition of domains, explaining why they behave similarly. In classification tasks, the average drops vary between 22 F1 points in ABSA to 2 F1 points in SA. In generation tasks models drop approximately 1.5 points of BERTScore in the AS and TG tasks.

It is worth examining the average worst SD and TD for the various tasks. As explained in \ref{sub:agg_metrics} these metrics show us the worst drop we can expect, averaged over all source or target domains. For example, even though the average drop in the SA task is 2 F1 points, for every source domain we can expect to find a harder transfer with a drop of 9 points on average.

This leads to the conclusion that the DR problem still exists in FT models across most tasks, though in a varying degree of severity. Some tasks (e.g. ABSA) exhibit significant drops in most domain transfers, while other tasks (e.g. QA) exhibit minor performance drops but can still expect to have harder transfers for every source domain.

In Appendix\ref{sec:additional_results} we study the effect of additional aspect of the DR of FT models, including model size, dataset size and number of epochs. We find that larger models tend to improve absolute in-domain and cross-domain performance, and in classification tasks also reduce the drop between them.

Few-shot models are much more robust to domain transfer. The drops are negligible, even having slightly negative ones (e.g. SA), with the worst tasks exhibiting drops of 0.5 or 1 points on average. This probably stems from the fact that few-shot learning imposes a weaker model anchoring in the source domain.

In Appendix \ref{sec:additional_results} we also study how the number of demonstrations affects DR, finding that a larger number of demonstrations usually improves in-domain and cross-domain performance, though in some cases mildly increasing the drop between them.

After seeing the extent of the DR problem in different tasks and setups, we wish to analyze how it manifests itself in the “real world”: How do the drops measure against the in-domain performance of the source and the target domains?

\subsection{Characterizing the DR Challenge}
\label{sub:characterizing}
To answer this question we study the distribution of the different DR scenarios discussed in \ref{sub:scenarios}.

The Classic DR challenge, which occurs when both the SD and the TD are positive, is the most common scenario. In fine-tuning classification tasks (and the AS task), over 70\% of the shifts exhibit the classic scenario. Notice that the four scenarios are prevalent in all of the few-shot learning tasks, and in that case, we may say that the effect of the domain shift is weak. It is also the case in the fine-tuning QA and QG tasks. 

The Unobserved DR challenge scenario (positive TD but negative SD) is common, occurring in 7 out of 8 FT tasks (ranging between 11\% in SA to 40\% in TG), and in all few-shot learning tasks occurring in noticeable proportions. This is an important observation since many of the past works overlooked the TD, focusing solely on the SD. Our study suggests that a DR challenge may exist (in terms of positive TD) even if participants do not observe a performance degradation. In comparison, the Observed DR challenge (positive SD but negative TD), is not as common as the Unobserved challenge, occurring in 4 out of the 8 fine-tuning tasks. This highlights the importance of providing an additional perspective (i.e., the TD) on performance degradation.

This calls for a deeper analysis: Which of these perspectives is a better estimator of the cross-domain performance?

\subsection{Comparing SD and TD}
\label{sub:comparing}

As discussed in \ref{sub:agg_metrics}, SD and TD share the same expectation, thus providing two unbiased estimators for the cross-domain performance ST. In \ref{tab:characterizing}, we see that for every task and for both fine-tuning and few-shot learning models, the variance of SD is larger than the variance of TD (except for the NLI task for few-shot learning), thus making him the noisier estimator. In addition, for almost all tasks the Average Worst SD is higher than the Average worst TD. This result indicates that the observed degradation attributed to domain shift in most DR works might not tell the whole story. 

A possible explanation could stem from the fact that the correlation between ST and TT is much stronger than the correlation with SS. For most fine-tuning tasks, it is above 0.8, while the correlation of SS with ST is relatively low. 

In conclusion, it is evident that estimating the cross-domain performance based solely on comparison to the SS will paint an obscure picture. A full picture can be obtained only by gaining some knowledge of the target's in-domain performance. This is infeasible in a realistic scenario, but further research can incorporate this viewpoint using our benchmark.

Few-shot learning is rapidly becoming a prominent paradigm in NLP. We've seen that few-shot models are more robust to domain transfer. Next, we would like to further compare them to fine-tuned models, in order to gain a better understanding of the effects of this trend on DR.

\subsection{Comparing Fine-Tuned and Few-Shot Models}
\label{sub:few_shot}

Few-shot are much more robust to domain transfer. As discussed in \ref{sub:dr_challenge}, they exhibit minor performance drops, possibly stemming from the fact that they are anchored to the source domain only by the demonstrations given and not by altering any parameters.

This robustness comes at a cost in terms of absolute performance, which varies between tasks. As seen in \ref{tab:main_fs_results}, for non-GPT models, the fine-tuned models beat all few-shot models, both in-domain and cross-domain. For the GPT models, aside from the AS task, the fine-tuned model is consistently better in-domain. In some tasks the fine-tuned model achieves a higher score also in cross-domain (NLI, QA, QG, TG), while in other tasks, the GPT models match the fine-tuned performance or beat it (SA, AB, AS).

To conclude, we have shown that the DR challenge persists in FT models across most tasks, though in varying degrees. Few-shot models are more robust but are outperformed by the FT models, though the gap is declining with SOTA models matching the FT models' performance in cross-domain. Taking into account also the target's in-domain performance, we see that in many cases there is an unobservable DR problem, while observable problems might be explained by transitions to harder domains. The target's in-domain performance is a better estimator of the cross-domain performance and has a very strong correlation with it, meaning that relying solely on the source's in-domain performance might paint a partial or even misleading picture.

==> 6.results_old.tex <==
\section{Results}
\label{sec:results}

% \input{tables/characterizing}

In this section, we present and discuss the results of our experiments. We start by characterizing the DR problem of fine-tuned models (\S\ref{sub:dr_problem}) and then provide an analysis of their performances (\S\ref{sub:fine_tuning}). Finally, in \S\ref{sub:zero_shot} we examine the stability of zero-shot and few-shot models and compare them to fine-tuned models.

\subsection{Characterizing the DR Problem}
\label{sub:dr_problem}

\input{tables/correlations}
\input{figures/triplet_barplot}

In this subsection, we aim to gain a deeper understanding of the differences between the tasks, which will help us characterize the DR problem and the behavior of the $\sd$ and the $\td$. To this end, we examine the relationship between the source and target in-domain performances ($\sss$ and $\ttt$) and the cross-domain performance ($\st$): We calculate the Spearman's correlation and the $L_1$ distance between $\st$ and $\sss$ and between $\st$ and $\ttt$. In addition, we compute the proportion of shifts with positive $\sd$ and $\td$. We present these results in Table~\ref{tab:correlations}. In Figure~\ref{fig:triplet} we examine the domain shift scenarios (see \S\ref{sub:scenarios}). Accordingly, we plot the proportion of each of the six possible performance orders within the $\triplet$ triplets.

\medskip\noindent\textbf{$\st$ behaves more like the $\ttt$ rather than $\sss$.} Table~\ref{tab:correlations} provides two interesting observations. The first is that the correlation between $\st$ and $\ttt$ is much stronger than the correlation with $\sss$, and for most tasks, it is above 0.8. The second is that the $\st$ scores are closer to $\ttt$ than to $\sss$ in terms of $L_1$ distance, which is not surprising since the two observations are equivalent according to Theorem~\ref{theorem:eq}. 

Accordingly, the $\ttt$ has much more influence on the $\st$ than the $\sss$. This result strengthens our argument that the target in-domain should be the  reference point when measuring a degradation, i.e., $\td$ is the right measure for DR, since fluctuations in $\sd$ may be caused by in-domain differences $\sss - \ttt$ and not with actual model robustness issues. \S\ref{sec:discussion} discusses further consequences of this finding.

Nevertheless, when the DR problem is severe, the target in-domain performance is not informative for the cross-domain performance. For example, the AE task, which has the highest degradation in performance (more than 20 F1 points) has the weakest correlation (0.11). In contrast, the strongest correlations (0.9 and 0.96) belong to the QA and QG tasks, which have the lowest degradation. 

\medskip\noindent\textbf{Source drop does not necessarily indicate a DR problem.} According to Table~\ref{tab:correlations} there is a majority of positive $\sd$ and $\td$ in all the tasks, indicating a DR problem exists, yet we ought to examine to which extent. Before we answer this in \S\ref{sub:fine_tuning}, we provide a few more interesting results on the relationship between $\sd$ and $\td$.  Figure~\ref{fig:triplet} shows that for the SA, NLI, AE, and AS tasks, the classic DR scenario (red bars) dominates: the $\st$ is smaller than both the $\ttt$ and $\sss$. Moreover, in the remaining scenarios there is still a DR problem, although it is unobservable ($\sss<\st<\ttt$). Our results show that the unobserved scenario is common.

In the QA, QG, and TG tasks, there is a large proportion of spurious DR scenarios: although there is an observed degradation, it does not stem from a real DR problem ($\ttt<\st<\sss$). This result highlights the importance of providing an additional perspective on the performance degradation (i.e., the $\td$). Furthermore, notice that in the QA and QG tasks, which share domains, there is a substantial proportion of scenarios with no degradation (blue bars). 

\subsection{Fine-tuning Performance Degradation}
\label{sub:fine_tuning}

In Figure~\ref{fig:abs_performance} we present in-domain ($\sss$) and cross-domain ($\st$) performances, including their average scores for every model and task. Figure~\ref{fig:drop_performance} shows the drops in the performance, including the average drop and the largest $\sd$ and $\td$ scores.

\input{figures/abs_performance}
\input{figures/drop_performance}

\medskip\noindent\textbf{In-domain performances are higher than cross-domain performances.} As shown in Figure~\ref{fig:abs_performance}, for all models, the average in-domain performance is higher than their cross-domain performance, except for the QA and QG tasks, where the difference between the two is minor.
The minor difference in the QA and QG, can be explained not only by a small drop, but by the no DR scenarios which counterbalance it.
Moreover, the magnitude of the average drop differs between the tasks. For example, DeBERTa-B exhibits an average drop of 3.45 on SA, a severe drop of 20.37 on AE, but only a 0.7 drop on QA. On Generation tasks, T5-B exhibits an average drop of 2.67 on TG and 1.625 on AS, and a small 0.3 drop on QG (see: Figure~\ref{fig:drop_performance}). Our results imply that the DR problem is still relevant to LMs. 

\medskip\noindent\textbf{Larger models improve performance, but not necessarily robustness.} Figure~\ref{fig:abs_performance} demonstrates that for most tasks, the general trend is that larger models of the same family improve in-domain and cross-domain performances. For example, DeBERTa-XS achieves F1 scores of 94.6 for in-domain and 91.0 for cross-domain, while DeBERTa-L improves these scores to 96.2 and 94.1, respectively. This results in an improvement of 1.5 on the average drop. There are a few exceptions to this positive trend, such as in the cases of DeBERTa on AE and T5 on TG, where the performance stays the same.

Regarding the performance drop, according to Figure~\ref{fig:drop_performance}, larger models seem to have no effect on the average drop, or at the very least, slightly minimize it (with the expectation of T5 on AS, where the drop modestly increases). Nevertheless, the average drop trends are weaker and less clear than the absolute in-domain and cross-domain trends. These findings are in line with \citet{transformers_improve_robustness} and prove them to be true on additional NLP tasks. 

% When comparing the different models on classification tasks, the DEBERTA models beat the ROBERTa models, having the \debertab perform approximately as the \robertal model. For example, on the SA task both achieve a 95.8 in-domain F-1 performance, but \debertab achieves an average of 93.6 cross domain while \robertal achieves only 92.7.

% For generation and QA tasks it is harder to conclude whether larger models always provide higher scores and lower DR drops. For example in Abstractive Summarization, we see that \tfivel{} \space has higher in-domain performance in comparison with \tfiveb, but lower cross-domain performance.

\medskip\noindent\textbf{The effect of the training size on DR.}

T.B.D


\medskip\noindent\textbf{Target Drop is smaller than Source Drop.} Another important finding is that the $\sd$ bigger than $\td$, as can be seen by the worst drops in Figure~\ref{fig:drop_performance}. Sometimes, the average worst $\sd$ is two to three times bigger (e.g., QG and TG). An exception is the SA task, where the worst $\td$ is bigger. 

This finding is not surprising, as our theorem suggests that the variance of $\sd$ is larger than the variance of $\td$, and intuitively, this means that the likelihood of observing a large value is higher (although without additional assumptions on the distributions, this cannot be theoretically proved). Moreover, our findings indicate that the degradation attributed to domain shift in the majority of DR works might be weaker than it is in practice. In \S\ref{sec:discussion}, we discuss the impact of this finding on DR research.

\medskip\noindent\textbf{There are challenging shifts in every task.} Finally, as can be seen by the worst $\sd$ and worst $\td$ lines in Figure~\ref{fig:drop_performance}, in every task and model, there is a substantial performance drop bigger than 5 points (with the expectation of the worst $\td$ for QA and QG). Accordingly, the large difference between the average and the worst drops suggests that synthetic domain shifts like challenge sets do not represent the average robustness of NLP models truthfully. On the other hand, the challenging shifts indicate that the DR problem is still relevant, even when the shift is natural and under simplifying assumptions (see \S\ref{tab:dataets}). Moreover, to facilitate further DR and DA research, we construct a benchmark that consists of only the challenging shifts. More details are provided in our project repository.

\subsection{Zero-shot and Few-shot}
\label{sub:zero_shot}



==> 7r.discussion_review.tex <==
\section{Extended Discussion}
\label{sec:extend_discussion}

In the section, we extend the discussion from \S\ref{sec:discussion} and summarise and discuss the key implications of our work.

\medskip\noindent\textbf{On Domain Robustness Research} 
As discussed in the paper, most past DR works focused solely on the observed performance degradation ($\sd$) as a measure of the DR challenge. However, as asserted in this paper, a full characterization of the DR challenge requires deriving the joint distribution of $\sss$, $\ttt$, and $\st$, which is not tractable. Therefore, we propose practical metrics to quantify the performance degradation: $\sd$ and $\td$. 

We need both metrics for a single domain shift because large drops might be attributed to the in-domain difference ($\idd$) and obscure the DR challenge of the shift. Indeed, our findings indicate that a large $\sd$ commonly coexists with a large $\idd$. At the task level, the expected values of both drop metrics ($\sd$ and $\td$) are equal and correspond to the average drop ($\drop$). However, we empirically find that the $\td$ is a better estimator of the $\drop$. This implies that when examining a limited number of domain shifts, it is crucial to include the $\td$. 
% The bottom line of this work is that a comprehensive assessment of the DR of NLP models requires following our proposed methodology: Evaluating multiple domain shifts for each task and incorporating both metrics. 

In addition, we suggest that current research may paint an inaccurate picture of the state of domain robustness. This stems from two of our findings. First, performance degradation is larger when measured with the $\sd$ than with the $\td$. Second, every task has shifts with severe performance drops, even when most shifts are not remotely as bad. 
This means that past works focused only on the $\sd$ and challenging shifts such as challenge sets and other highly-curated datasets present a distorted image of the actual state of DR, which is actually much milder. Nevertheless, we acknowledge the importance of challenge sets as diagnostic tools. 

\medskip\noindent\textbf{On the Relevance of Fine-tuning} 
Zero-shot and few-shot LLMs can perform various tasks without the additional cost of annotating data or training a model. However, their usage can be very costly, as they require massive computational resources, and their latency can be extremely high. Additionally, when the data cannot be sent to external servers because of privacy constraints or when the domain is unique or specific (e.g., in national security settings or human conversations), LLMs that cannot be fine-tuned may be less effective. Moreover, with enough task-specific labeled data that few-shot LLMs can cheaply annotate, it is possible to develop a small, high-performing, fine-tuned model \citep{kd_nlg, TrueTeacher, comblm}. For these reasons, fine-tuning a smaller model that does not have few-shot capabilities is still the de-facto standard \citep{standing_on}.

% Despite the advantages of few-shot LLMs, several works have demonstrated that fine-tuning LLMs on specific downstream tasks outperform few-shot LLMs \citep{alexa, ul2}, even when the latter are much larger. 
Moreover, there is strong evidence that few-shot language models underperform fine-tuned models in specific domains that require expertise, such as biomedical \citep{gpt3_biomedical} or when the training size is large enough \citep{revisiting}. This study also shows that task-specific fine-tuned models outperform few-shot models in-domain, although this gap may be closed soon. Nevertheless, we also found that few-shot LLMs are more robust to domain shifts and can outperform fine-tuned models cross-domain. This calls for further Domain Adaptation research of fine-tuned models. 

% \input{tables/challenge_shifts}

\medskip\noindent\textbf{On the Relevance of Domain Adaptation} 
Domain Adaptation (DA) is a field that addresses solutions to the DR problem. DA research considers various setups, each having different assumptions on the availability of data from the target domain at the model training time \citep{sentiment_blitzer, da_data_selection, ziser1, ziser3, self_training_rotman, perl, unsupervised_da_survey, adapters, pada, docogen, hyperpada, da_prompts, da_la23, da_li23, da_va23}. 

Modern NLP models are believed to be robust due to the pretraining process, where the models have seen a vast amount of diverse data from various domains. Another reason could be data contamination \citep{contamination, contamination2}, i.e., pretraining on data from a downstream task improves the performance on it \citep{gpt2, dg_continue_pretraining_classification, continue_pretraining_for_da}. This belief questions the relevance or the necessity of Domain Adaptation research.

However, in this study, we demonstrated that the DR challenge still exists. We show that there is a performance drop due to domain shift in every task or model, and moreover, some shifts are remarkably challenging. We believe that DA research remains essential and relevant, particularly for NLP. To facilitate further research, we provide an NLP benchmark with natural topic shifts, which has some challenging setups for various NLP tasks. We hope this benchmark will be used to evaluate and improve DA methods.

\medskip\noindent\textbf{On Predicting Cross-domain Performance} Estimating performance has an important impact on the deployment and maintenance of NLP models and related financial decisions (e.g., the need for annotation) \citep{predict_dr2, predict_dr1, predict_no_asnwer, al_da}. We found that the $\ttt$ is a better predictor of the cross-domain performance ($\st$) than the $\sss$. Accordingly, knowledge about the target domain is essential, and without it, estimators may struggle to predict cross-domain performance. In addition, previous studies have attempted to predict performance drops (specifically, only the $\sd$) using domain divergence \citep{divergence_survey}. Our study (see \ref{sub:divergence}) suggests that domain divergence is a better predictor of the $\td$ than the $\sd$.

% \medskip In conclusion, our comprehensive study of Domain Robustness in NLP models highlights the need for a nuanced approach in assessing their performance across domain shifts. We have advocated that current research can paint a skewed picture of NLP models' robustness. This work underscores the ongoing relevance of Domain Adaptation research in NLP and the importance of developing robust, adaptable models capable of handling the diverse nature of real-world data.


==> figures/drops_intro_tex.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/drops_intro_.pdf}
    \caption{Domain shift from source domain $S$ to target domain $T$. The black square ($\sss$) is the source in-domain performance (training and evaluating on $S$). The green diamond ($\st$) is the cross-domain performance (training on $S$ and evaluating on $T$). The grey circle ($\ttt$) is the target in-domain performance (training and evaluating on $T$).
    We observe a 10\% performance drop when shifting from $S$ to $T$ ($SS=80\%$ and $ST=70\%$). In this case we would typically conclude that there is a Domain Robustness (DR) challenge.
    However, had we \emph{hypothetically} trained and tested the model on data from $T$, its target in-domain performance would be $65\%$ ($\ttt$), which indicates that the model actually gains $+5\%$ when trained on $S$, in comparison to $T$. 
    Most DR works consider only the \emph{observed} Source Drop ($\sd = \sss - \st$) and ignore the \emph{hidden} Target Drop ($\td = \ttt - \st$), resulting in a partial depiction of the DR challenge.}
    % \caption{A domain shift example from the source domain A (notated as $S$) to the target domain B (notated as $T$). The black square, $\sss$ (=80\%), is the source in-domain performance (testing on $S$). The green diamond, $\st$ (=70\%) is the cross-domain performance (a.k.a OOD performance, testing on $T$). We may say there is a Domain Robustness (DR) challenge since we observe a 10\% performance drop. However, had we hypothetically trained and tested the model on data from $T$, its target in-domain performance ($\ttt$, grey circle) would be 65\%, meaning the model gains 5\% when trained on $S$, in comparison to $T$. Most DR works consider only the \emph{observed} Source Drop ($\sd = \sss - \st$) and ignore the \emph{unobserved} Target Drop ($\td = \ttt - \st$), resulting in a partial depiction of the DR challenge.}
    \label{fig:drops_intro}
\end{figure}

==> figures/drops_vis_tex.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/drops_viz.pdf}
    \caption{Our running example of domain shifts involving three domains: A, B and C. Black dashed horizontal lines represent in-domain performance. Short green lines represent cross-domain performance. Orange arrows represent $\sd$s, and blue arrows represent $\td$s.
    }
    \label{fig:drops_vis}
\end{figure}

==> figures/fs_demons_main_tex.tex <==
\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\textwidth]{figures/fs_GPT3.5_performance.pdf}
    \includegraphics[width=\textwidth]{figures/fs_GPT3.5_drop.pdf}
    \caption{Performance (top) and drops (bottom) of GPT3.5 as a function of the number of few-shot demonstrations. The top plot presents the F1 and BertScore scores of the average in-domain (black line) and cross-domain (green line) performance. In addition, the highest in-domain score (orange line) and the lowest cross-domain score (blue line) are displayed. The bottom plot presents the Average Drop (green line), The Worst $\sd$ (orange line), and the Worst $\td$ (blue line). }
    \label{fig:demons_gpt_main}
\end{figure*}


==> figures/intro_figure_tex.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.44\textwidth]{figures/intro_figure.pdf}
    \caption{Illustration of three scenarios of the DR challenge and the main concepts we use in our work. The horizontal orange lines represent the in-domain performance ($\sss$). For example, the performance of the NLP model is 90 when training and evaluating it on domain $A$ ($A \rightarrow A$). The cross-domain performance is $\st$ (green lines), and although it equals 75 in all three scenarios, the DR challenge is different. Consider the middle column with the domain shift $A \rightarrow C$, where we observe a 15-point drop from the in-domain performance. In this case, we would typically conclude that there is a DR challenge. However, had we trained and tested the model on data from $C$, its target in-domain performance ($\ttt$, blue lines) would be 70, suggesting an actual 5-point improvement when trained on $A$ compared to $C$. Unlike the ``Observed'' scenario in the middle, in the left ``Classic'' scenario ($A \rightarrow B$) the $\st$ is lower than both $\sss$ and $\ttt$, aligning with typical expectations of a DR challenge.
    Most works focus solely on the Source Drop ($\sd = \sss - \st$) and overlook the Target Drop ($\td = \ttt - \st$), resulting in a partial depiction of the DR challenge. In this study, we provide a fresh perspective by also considering the $\td$, revealing that while nuanced, the DR challenge in NLP is still prevalent.}
    \label{fig:intro}
    \vspace{-0.5em}
\end{figure}


% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.44\textwidth]{figures/intro_figure.pdf}
%     \caption{Illustration of three scenarios of the DR challenge and the main concepts we use in our work. The horizontal orange lines represent the in-domain performance ($\sss$). For example, the performance of the NLP model is 90 when training and evaluating it on domain $A$ ($A \rightarrow A$). The cross-domain performance is $\st$ (green lines), and although it equals 75 in all three scenarios, the DR challenge is different. Consider the middle column with the domain shift $A \rightarrow C$, where we observe a 15-point drop from the in-domain performance. In this case, we would typically conclude that there is a DR challenge. However, had we trained and tested the model on data from $C$, its target in-domain performance ($\ttt$, blue lines) would be 70, suggesting an actual 5-point improvement when trained on $A$ compared to $C$. Unlike the ``Observed'' scenario in the middle, the left scenario ($A \rightarrow B$) is termed ``Classic'', as $\st$ is lower than both $\sss$ and $\ttt$, aligning with typical expectations of a DR challenge.
%     Most works focus solely on the \textit{observed} Source Drop ($\sd = \sss - \st$) and overlook the \textit{unobserved} Target Drop ($\td = \ttt - \st$), resulting in a partial depiction of the DR challenge. In this study, we provide a fresh perspective by also considering the $\td$, revealing that while nuanced, the DR challenge in modern NLP models is still prevalent.}
%     \label{fig:intro}
%     \vspace{-0.5em}
% \end{figure}

==> tables/challenge_shifts.tex <==
\begin{table}
\centering
\large
\begin{adjustbox}{width=0.47\textwidth}
\begin{tabular}{l|ll|ccccc}
\hline
\textbf{Task} & \textbf{Source} & \textbf{Target} & \textbf{$\sss$} & \textbf{$\st$} & \textbf{$\ttt$} & \textbf{$\sd$} & \textbf{$\td$} 
\\
\hline
SA   &        Airline &         Books &  91.7 &  87.5 &  97.7 &   4.3 &  10.2 \\
NLI  &         Travel &     Telephone &  90.1 &  82.0 &  87.7 &   8.1 &   5.7 \\
AE   &         Device &          mams &  74.6 &  37.6 &  73.8 &  37.0 &  36.2 \\
QA   &      Geography &       Science &  80.4 &  75.9 &  79.0 &   4.4 &   3.1 \\
\hline
QG   &           Tech &       History &  50.7 &  44.0 &  45.2 &   6.7 &   1.2 \\
AS   &  Relationships &           LoL &  26.0 &  19.0 &  20.7 &   7.1 &   1.7 \\
TG   &         Beauty &         Books &  39.6 &  27.6 &  29.8 &  11.9 &   2.2 \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Performance and drops for the DA benchmark, consisting of a single challenge domain shift for each task. The table presents the F1 scores of DeBERTa-L for the classification and the QA tasks, and the ROUGE-L F1 scores of T5-L for the generation tasks.}
\label{tab:challenge}
\end{table}

==> tables/main_table_ft_vs_fs.tex <==
\begin{table}[t]
\centering
% \footnotesize
\begin{adjustbox}{width=0.44\textwidth}
\begin{tabular}{l|l|ccccc}
\toprule
\textbf{Task} & \textbf{Model} & {\footnotesize $\overline{\sss}$ } & {\footnotesize $\overline{\st}$ } & {\footnotesize $\drop$ } & {\footnotesize $W_{\sd}$ } & {\footnotesize $W_{\td}$ } \\
\midrule
  \multirowcell{2}{SA} & DeBERTa-L &           \textbf{96.2} &              94.1 &       2.1 &      \textbf{9.6} &     \textbf{10.2} \\
  & GPT4 &              95.2 &        \textbf{94.7} &  \textbf{0.5}  &     11.0 &           \textbf{2.0} \\
\hline
 \multirowcell{2}{NLI} & DeBERTa-L &           \textbf{90.4} &              \textbf{88.9} &       1.5 &      5.4 &      3.1 \\
   & GPT4 &  87.0 &                  86.0 &  \textbf{1.0} &       6.4 &          3.9  \\
\hline
  \multirowcell{2}{AB} & RoBERTa-L &           \textbf{73.3} &              \textbf{49.4} &      23.9 &     35.2 &     32.4 \\
   & GPT4 & 51.0 &                 47.9 &  \textbf{3.1} &       \textbf{28.9} &          \textbf{6.9}  \\
\hline
  \multirowcell{2}{QA} & RoBERTa-L &           \textbf{82.0} &              \textbf{81.7} &      0.3 &      \textbf{6.0} &      2.5 \\
   & GPT4 & 71.0 &                 71.1 &     \textbf{-0.1} &     \textbf{6.0} & \textbf{0.8} \\
\hline
  \multirowcell{2}{QG} &      T5-L &           \textbf{77.3} &              \textbf{77.2} &       \textbf{0.1} &      4.3 &      1.2 \\
      & GPT4 &  76.0 &                 75.8 &   0.2 &      \textbf{3.5} &          \textbf{0.5} \\ 
\hline
  \multirowcell{2}{AS} &      T5-L &           62.4 &              61.4 &       1.0 &      4.6 &      2.5 \\
        & GPT4 & \textbf{64.1} &                 \textbf{64.0} & \textbf{0.1}    &     \textbf{2.5} & \textbf{0.6} \\
\hline
  \multirowcell{2}{TG} &      T5-L &           \textbf{66.5} &              \textbf{65.2} &       1.3 &      6.8 &      5.1 \\
   & GPT4 & 58.0 &                 57.9 &  \textbf{0.1} &       \textbf{1.5} & \textbf{0.4} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Comparison between fine-tuned and few-shot models. The columns are: $\overline{\sss}$ - Average In-domain Performance, $\overline{\st}$ - Average Cross-domain Performance, $\drop$ - Average Drop, $W_{\sd}$ - Worst Source Drop and $W_{\td}$ - Worst Target Drop.}
\label{tab:main_ft}
\vspace{-0.5em}
\end{table}

==> tables/models.tex <==
\begin{table}
\centering
\footnotesize
\begin{adjustbox}{width=0.4\textwidth}
\begin{tabular}{lcccl}
\toprule
\textbf{Name} & \textbf{Arch.} & \textbf{Params} & \textbf{Layers} & \textbf{Open}\\
\midrule
DistilBert & \multirowcell{3}{EO} & 66m & 6 & \multirowcell{3}{Yes} \\
RoBERTa-B &  & 125m & 12 &  \\
RoBERTa-L &  & 355m & 24 &  \\
\midrule
DeBERTa-XS & \multirowcell{4}{EO} & 70m & 12 & \multirowcell{4}{Yes} \\
DeBERTa-S &  & 142m & 6 &    \\
DeBERTa-B &  & 184m & 12 &   \\
DeBERTa-L &  & 435m & 24 &   \\
\midrule
T5-S & \multirowcell{3}{ED} & 60m & 12 & \multirowcell{3}{Yes} \\
T5-B &  & 220m & 24 &  \\
T5-L &  & 737m & 48 &  \\
\midrule
BART-B & \multirowcell{2}{ED} & 139m & 12 & \multirowcell{2}{Yes} \\
BART-L &  & 406m & 24 &  \\
\midrule
Orca 7b & \multirowcell{2}{DO} & 7b & 32 & \multirowcell{2}{Yes} \\
Orca 13 &  & 13b & 40 &  \\
\midrule
Mistral 7b & \multirowcell{2}{DO} & 7b & 32 & \multirowcell{2}{Yes} \\
NeuralChat &  & 7b & 32 &  \\
\midrule
GPT3.5 & \multirowcell{2}{DO} & \multirowcell{2}{?} & \multirowcell{2}{?} & \multirowcell{2}{No} \\
GPT4 &  &  &  &  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Details about the participating models in this study. 
``Arch.'' states the architecture type: EO for Encoder-only, ED for Encoder-decoder, and DO for Decoder-only. Notice that EO and ED models are fine-tuned, while DO models are used in few-shot setups.
``Params'' is the number of parameters in millions (m) or billions (b).
``Layers'' is the number of layers. ``Open'' states whether the model is open-sourced.}
\label{tab:models}
\vspace{-0.5em}
\end{table}
